An Evaluation of Three Distance Measurement Technologies for Flying Light Specks

This study evaluates the accuracy of three different types of time-of-flight sensors to measure distance. We envision the possible use of these sensors to localize swarms of flying light specks (FLSs) to illuminate objects and avatars of a metaverse. An FLS is a miniature-sized drone configured with RGB light sources. It is unable to illuminate a point cloud by itself. However, the inter-FLS relationship effect of an organizational framework will compensate for the simplicity of each individual FLS, enabling a swarm of cooperating FLSs to illuminate complex shapes and render haptic interactions. Distance between FLSs is an important criterion of the inter-FLS relationship. We consider sensors that use radio frequency (UWB), infrared light (IR), and sound (ultrasonic) to quantify this metric. Obtained results show only one sensor is able to measure distances as small as 1 cm with a high accuracy. A sensor may require a calibration process that impacts its accuracy in measuring distance.

==> infrared.tex <==
\section{Infrared}\label{sec:IR}

%\begin{figure*}[!ht]
\begin{figure*}
\centering
\begin{subfigure}[t]{0.47\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figs/SparkFunLow.jpg}
  \caption{IR sensor is touching the sheet.}
  %%%\label{fig:write_around}
\end{subfigure}
\quad
\begin{subfigure}[t]{0.47\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figs/SparkFunElevated.png}
  \caption{IR sensor is elevated 3.7 cm.}
  %%%\label{fig:write_through}
\end{subfigure}
\caption{Elevation impacts accuracy of measured distances with IR.}
\label{fig:infrared}
\end{figure*}

%\begin{itemize}
%    \item How does it work? 
%    \item What are its theoretical/physical limits?
%    \item How did we do the evaluation?  Show pictures.
%    \item What are our interesting finds?
%\end{itemize}

Infrared (IR) sensors are active sensors that emit a signal (IR light) and then detect the signal's return after it bounces off of the object. The sensor calculates the distance to the object using the time-of-flight (i.e., the amount of time recorded between emitting and detecting the light):
\begin{equation}
    d=v_lt/2
\end{equation}
where $v_l$ is the speed of light and $t$ is the recorded time.

IR sensors can sense closer objects and have a higher resolution than ultrasonic sensors, but they have an overall shorter range. A typical IR sensor has a range of 0--130 cm with a resolution of 1 mm~\cite{benet2002using}.
However, this range can be affected by the color of the object it is detecting. While color does not change the amount of time it takes for the light to travel, lighter colors reflect more light than darker colors. Therefore, the sensor's optimal distance range will be when detecting white objects (i.e., reflecting most light) and its worst distance range will be when detecting black objects (i.e., reflecting least light). 

The wavelength of IR sensors (940 nm) is also significantly less than that of ultrasonic sensors, meaning that they can detect significantly smaller objects than ultrasonic sensors~\cite{benet2002using}. This parameter is very important in FLS systems. IR sensors also have a smaller FoV (18$^\circ$) than ultrasonic sensors, creating a higher spatial resolution.

One limitation of IR sensors is that their performance can be affected by external light in the environment. Significant IR light from the environment can saturate the sensor or cause incorrect distance readings. Therefore, these sensors are more accurate indoors than outdoors. Best practices with IR sensors includes shielding the sensor from external light to mitigate any errors.

 

\begin{figure*}
\centering
\begin{subfigure}[t]{0.31\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figs/Sparkfun 1cm Distances Non-Elevated New Colors.png}
  \caption{IR sensor is touching the sheet.  Measuring different distances with a 1 cm calibration.}\label{fig:infraredTouching}
  %%%\label{fig:write_around}
\end{subfigure}
\quad
\begin{subfigure}[t]{0.31\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figs/SF1cmDistancesElevated_AdjustedYAxis.png}
  \caption{IR sensor is elevated 3.7 cm.  Measuring different distances with a 1 cm calibration.}\label{fig:infraredElevated}
\end{subfigure}
\quad
\begin{subfigure}[t]{0.31\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figs/SF121020wRespectiveCalibrations.png}
  \caption{Percentage error in measuring 1 cm with 1 cm calibration, 2 cm with 2 cm calibration, 10 cm with 10 cm calibration, and 20 cm with 20 cm calibration.}\label{fig:IRaltcalib}
\end{subfigure}
\caption{IR quantifying different distances using alternative calibrations.}
\label{fig:infraredError}
\end{figure*}

With IR, we considered two experimental setups:  sensor closest to the table and sensor raised 3.7 cm above the table.
See Figure~\ref{fig:infrared}.
Figures~\ref{fig:infraredTouching} and~\ref{fig:infraredElevated} show the accuracy of measuring different distances with a 1 cm calibration for the two setups, respectively.
%distances using different calibrations of 1, 2, 10, and 20 cm for the two setups, respectively.
%we observed its accuracy is impacted by whether the sensor was elevated or not, see Figure~\ref{fig:infrared}.
%Figures~\ref{fig:infraredTouching} and~\ref{fig:infraredElevated} show the accuracy of measuring 1 cm distances using different calibrations of 1, 2, 10, and 20 cm.
The accuracy is highest when measuring distances of 1 or 2 cm.  The percentage error is higher with 10 and 20 cm.
With 20 cm measurements, the elevated setup provides a lower error.
Note that the scale of the y-axis is log in Figure~\ref{fig:infraredTouching}.
%the sensor/drone elevated 3.7 cm.  The error increases dramatically as the sensor is closer to the table, impacting greater distances the most.
Conceptually, this is due to the 3D cone shape of the sensor that is blocked by the table.
%Note that the amount of error (length of error bars) is significantly smaller when the sensor is elevated.
We anticipate the sensors to be mounted on the FLSs and the FLSs to fly at least a few centimeters above the ground.
Hence, the results of Figure~\ref{fig:infraredElevated} are most applicable. 

Similar to UWB, IR measures a distance more accurately when it is calibrated for the distance. 
Figure~\ref{fig:IRaltcalib} shows this and an enhanced accuracy with longer distances.
The average percentage error is close to 0\% with 2, 10, and 20 cm.
We were not able to calibrate IR to measure a 100 cm distance.


